Identifying Implementation Bugs in Machine Learning based Image Classifiers using Metamorphic Testing

We have recently witnessed tremendous success of Machine Learning (ML) in practical applications. Computer vision, speech recognition and language translation have all seen a near human level performance. We expect, in the near future, most business applications will have some form of ML. However, testing such applications is extremely challenging and would be very expensive if we follow today's methodologies. In this work, we present an articulation of the challenges in testing ML based applications. We then present our solution approach, based on the concept of Metamorphic Testing, which aims to identify implementation bugs in ML based image classifiers. We have developed metamorphic relations for an application based on Support Vector Machine and a Deep Learning based application. Empirical validation showed that our approach was able to catch 71% of the implementation bugs in the ML applications.

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c116/Testing/5Epochs/sedR2y72w <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 116 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c116/Testing/5Epochs/sedVmYE6Y <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 116 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c116/Training/150Epochs/sed3cNI1R <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 116 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c116/Training/150Epochs/sedDA1eZ7 <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 116 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c116/Training/150Epochs/sedlmjmgD <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 116 150 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c116/Training/150Epochs/sedqZeq5Y <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant  5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c116/Training/150Epochs/sedqa7TBr <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 116 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c116/Training/150Epochs/sedu8CprY <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 116 150 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c116/Training/5Epochs/sed9lyy0B <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 116 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c116/Training/5Epochs/sedQRNnjf <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 116 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c116/Training/5Epochs/sedVncnlT <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 116 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c116/Training/5Epochs/sedpQnI0q <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 116 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c116/Training/5Epochs/sedyspDGJ <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 116 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c221/Testing/5Epochs/sedCulBad <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 221 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c221/Testing/5Epochs/seddwMDmY <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 221 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c221/Training/150Epochs/sedBEVQWd <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 221 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c221/Training/150Epochs/sedEhtXqR <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 221 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c221/Training/150Epochs/sedHVaa55 <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 221 150 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c221/Training/150Epochs/sedKPEqln <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 221 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c221/Training/150Epochs/sedLsfm8b <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 221 150 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c221/Training/5Epochs/sed7yq65T <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 221 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c221/Training/5Epochs/sedcsLP5b <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 221 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c221/Training/5Epochs/sedkLQYHE <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 221 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c221/Training/5Epochs/sedwzAAu9 <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 221 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c221/Training/5Epochs/sedx0y732 <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 221 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c29/Testing/5Epochs/sedCG3uDG <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 29 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c29/Testing/5Epochs/sedcrzyih <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 29 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c30/Testing/5Epochs/sedsfRCl6 <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 30 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c30/Testing/5Epochs/sedwP14IF <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 30 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c31/Testing/5Epochs/sedbqaJbE <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 31 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c31/Testing/5Epochs/sedrsqnBc <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 31 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c32/Testing/150Epochs/sedHITUBU <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 32 150Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c32/Testing/150Epochs/sedvccDSb <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 32 150Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c32/Testing/5Epochs/sedTMxOA1 <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 32 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c32/Testing/5Epochs/sedjGctjI <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 32 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c33/Testing/5Epochs/sed7heKD4 <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 33 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c33/Testing/5Epochs/sed8jD2Ff <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 33 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c34/Testing/5Epochs/sed2KPghh <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 34 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c34/Testing/5Epochs/sedadKcCG <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 34 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c35/Testing/5Epochs/sedOLVmKK <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 35 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c35/Testing/5Epochs/sedijJsV8 <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 35 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c35/Training/150Epochs/sed4j3yGT <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 35 150 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c35/Training/150Epochs/sedJQ51WF <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 35 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c35/Training/150Epochs/sedR1X7ni <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 35 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c35/Training/150Epochs/sedmJZCXg <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 35 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c35/Training/150Epochs/sedzJ0oPZ <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 35 150 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c36/Testing/5Epochs/sed20ISif <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 36 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c36/Testing/5Epochs/sedzbeKZn <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 36 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c43/Training/5Epochs/sedYFmbey <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 43 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c43/Training/5Epochs/sedbFB34h <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 43 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c43/Training/5Epochs/sedxHDsbT <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 43 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c43/Training/5Epochs/sedxWv8c8 <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 43 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c43/Training/5Epochs/sedxqrWjr <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 43 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c44/Testing/5Epochs/sedVwZBXb <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 44 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c44/Testing/5Epochs/sedtSqM2j <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 44 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c44/Training/150Epochs/sedBNftCi <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 44 150 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c44/Training/150Epochs/sedeW3MQ0 <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 44 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c44/Training/150Epochs/sedq36DtE <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 44 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c44/Training/150Epochs/sedsRc8DC <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 44 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c44/Training/150Epochs/sedyEY4Tf <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 44 150 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c44/Training/5Epochs/sedEDVSdM <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 44 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c44/Training/5Epochs/sedQDWKyo <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 44 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c44/Training/5Epochs/sedUx8GdX <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 44 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c44/Training/5Epochs/sedcoAI6l <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 44 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c44/Training/5Epochs/sedrzVg3a <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 44 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c45/Testing/5Epochs/sedG6RXHM <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 45 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c45/Testing/5Epochs/sedq0UJ4x <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 45 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c45/Training/150Epochs/sed82GfIN <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 45 150 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c45/Training/150Epochs/sedMALRA5 <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 45 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c45/Training/150Epochs/sedO0Z5b3 <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 45 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c45/Training/150Epochs/sedlFKKmH <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 45 150 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c45/Training/150Epochs/sedt3Jchh <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 45 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c45/Training/5Epochs/sed8wRZqU <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 45 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c45/Training/5Epochs/sedFTvdGz <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 45 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c45/Training/5Epochs/sedKS8DKg <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 45 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c45/Training/5Epochs/seduSNHGy <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 45 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c45/Training/5Epochs/seduZT10R <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 45 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c49/Testing/5Epochs/sed25BFOY <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 49 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c49/Testing/5Epochs/sedsnmGId <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 49 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c49/Training/5Epochs/sed1MLCFT <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 49 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c49/Training/5Epochs/sed1mZbEt <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 49 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c49/Training/5Epochs/sed3exzBe <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 49 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c49/Training/5Epochs/sedCSqT9Z <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 49 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c49/Training/5Epochs/sedYVsWPh <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 49 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c50/Testing/5Epochs/sedTKVMOr <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 50 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c50/Testing/5Epochs/sedzOuGwd <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 50 5Epochs'
set xlabel 'step'
set ylabel 'validation loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:2 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 4:5 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 7:8 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 10:11 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 13:14 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 16:17 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c50/Training/150Epochs/sedfub8CK <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 50 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c50/Training/150Epochs/sedoKthmn <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 50 150 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c50/Training/150Epochs/sedpdkR2Z <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 50 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c50/Training/150Epochs/sedvqy7fx <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 50 150 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c50/Training/150Epochs/sedxgbizP <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 50 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c50/Training/5Epochs/sedAugzkb <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 50 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c50/Training/5Epochs/sedDUQ8GS <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 50 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [*:*:1]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c50/Training/5Epochs/sedRwSWiE <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 50 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c50/Training/5Epochs/sedXcxBKv <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 50 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/c50/Training/5Epochs/sedhZ83zl <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 50 5 Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


set xrange [*:3600]
set yrange [0:3]
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/r48/Training/150Epochs/sed3BThl1 <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 48 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/r48/Training/5Epochs/sedPYwAVO <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 48 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/r49/Training/150Epochs/sedQuV5Ui <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 49 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/r49/Training/5Epochs/sedBXxt5f <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 49 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/r6/Training/150Epochs/sedfeZbkA <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 6 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/r6/Training/5Epochs/sedLOc2mq <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 6 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/r67/Training/150Epochs/sedebsQDN <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 67 150Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/Mutants/MR1-permutingRGB/r67/Training/5Epochs/sedsKvrZt <==
set terminal wxt
set key font "courier,10"
set key noenhanced
set datafile separator ","
set title 'MR1 Mutant 67 5Epochs'
set xlabel 'step'
set ylabel 'training loss'
set key autotitle columnheader 
set key below maxcols 3 height 3
set colors classic

set for[i=1:10] linetype i dashtype  1


#set xrange [*:*]
set autoscale x
#set yrange [*:*]
set autoscale y
set ytics 0.5
plot 'combinedData.csv' using 1:3 w lp lw 2 lt 1 pt 2  ps 1.25 lc 0,\
     'combinedData.csv' using 5:7 w  lp lw 2 lt 2 pt 4  ps 1.25 lc 1,\
	 'combinedData.csv' using 9:11 w lp lw 2 lt 3 pt 6  ps 1.25 lc 3,\
	 'combinedData.csv' using 13:15 w lp lw 2  lt 4 pt 5  ps 1.25 lc 2,\
	 'combinedData.csv' using 17:19 w lp lw 2 lt 5 pt 12  ps 1.25  lc 7,\
	 'combinedData.csv' using 21:23 w lp lw 2 lt 6 pt 1  ps 1.25  lc 4

==> figures/results/CNNs/RESNET/Cifar10/OrigCode_(nonBuggy)/MR1-permutingRGB/Training/5Epochs/logs_MR1_BRG_5epochs <==
INFO:tensorflow:Using config: {'_task_type': 'worker', '_save_checkpoints_steps': None, '_session_config': None, '_service': None, '_save_checkpoints_secs': 1000000000.0, '_num_ps_replicas': 0, '_master': '', '_is_chief': True, '_tf_random_seed': 7, '_num_worker_replicas': 1, '_cluster_spec': <tensorflow.python.training.server_lib.ClusterSpec object at 0x000001911CA7F9B0>, '_log_step_count_steps': 100, '_keep_checkpoint_every_n_hours': 10000, '_task_id': 0, '_save_summary_steps': 100, '_model_dir': 'cifar10_model', '_keep_checkpoint_max': 5}
WARNING:tensorflow:From codeWithMRs/MR1-changeRGB/cifar10_main_VERML_basedOn_nas_fix4_deterministic_brg.py:87: FixedLengthRecordDataset.__init__ (from tensorflow.contrib.data.python.ops.readers) is deprecated and will be removed in a future version.
Instructions for updating:
Use `tf.data.FixedLengthRecordDataset`.
WARNING:tensorflow:From codeWithMRs/MR1-changeRGB/cifar10_main_VERML_basedOn_nas_fix4_deterministic_brg.py:166: calling Dataset.map (from tensorflow.contrib.data.python.ops.dataset_ops) with output_buffer_size is deprecated and will be removed in a future version.
Instructions for updating:
Replace `num_threads=T` with `num_parallel_calls=T`. Replace `output_buffer_size=N` with `ds.prefetch(N)` on the returned dataset.
WARNING:tensorflow:From codeWithMRs/MR1-changeRGB/cifar10_main_VERML_basedOn_nas_fix4_deterministic_brg.py:166: calling Dataset.map (from tensorflow.contrib.data.python.ops.dataset_ops) with num_threads is deprecated and will be removed in a future version.
Instructions for updating:
Replace `num_threads=T` with `num_parallel_calls=T`. Replace `output_buffer_size=N` with `ds.prefetch(N)` on the returned dataset.
INFO:tensorflow:Create CheckpointSaverHook.
INFO:tensorflow:Saving checkpoints for 1 into cifar10_model\model.ckpt.
INFO:tensorflow:train_accuracy = 0.0703125, cross_entropy = 2.6708, learning_rate = 0.1
INFO:tensorflow:step = 1, loss = 2.88288
INFO:tensorflow:Saving checkpoints for 40 into cifar10_model\model.ckpt.
INFO:tensorflow:Loss for final step: 2.22981.
INFO:tensorflow:Starting evaluation at 2017-12-12-01:16:09
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-40
INFO:tensorflow:Finished evaluation at 2017-12-12-01:16:18
INFO:tensorflow:Saving dict for global step 40: accuracy = 0.10297, global_step = 40, loss = 58.0359
INFO:tensorflow:Create CheckpointSaverHook.
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-40
INFO:tensorflow:Saving checkpoints for 41 into cifar10_model\model.ckpt.
INFO:tensorflow:train_accuracy = 0.351563, cross_entropy = 1.78381, learning_rate = 0.1
INFO:tensorflow:step = 41, loss = 1.99728
INFO:tensorflow:Saving checkpoints for 80 into cifar10_model\model.ckpt.
INFO:tensorflow:Loss for final step: 2.01516.
INFO:tensorflow:Starting evaluation at 2017-12-12-01:19:25
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-80
INFO:tensorflow:Finished evaluation at 2017-12-12-01:19:34
INFO:tensorflow:Saving dict for global step 80: accuracy = 0.10396, global_step = 80, loss = 14.2363
INFO:tensorflow:Create CheckpointSaverHook.
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-80
INFO:tensorflow:Saving checkpoints for 81 into cifar10_model\model.ckpt.
INFO:tensorflow:train_accuracy = 0.382813, cross_entropy = 1.64169, learning_rate = 0.1
INFO:tensorflow:step = 81, loss = 1.85508
INFO:tensorflow:Saving checkpoints for 120 into cifar10_model\model.ckpt.
INFO:tensorflow:Loss for final step: 1.96434.
INFO:tensorflow:Starting evaluation at 2017-12-12-01:22:39
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-120
INFO:tensorflow:Finished evaluation at 2017-12-12-01:22:48
INFO:tensorflow:Saving dict for global step 120: accuracy = 0.0960396, global_step = 120, loss = 6.88776
INFO:tensorflow:Create CheckpointSaverHook.
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-120
INFO:tensorflow:Saving checkpoints for 121 into cifar10_model\model.ckpt.
INFO:tensorflow:train_accuracy = 0.421875, cross_entropy = 1.51403, learning_rate = 0.1
INFO:tensorflow:step = 121, loss = 1.7268
INFO:tensorflow:Saving checkpoints for 160 into cifar10_model\model.ckpt.
INFO:tensorflow:Loss for final step: 1.68123.
INFO:tensorflow:Starting evaluation at 2017-12-12-01:25:52
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-160
INFO:tensorflow:Finished evaluation at 2017-12-12-01:26:01
INFO:tensorflow:Saving dict for global step 160: accuracy = 0.130693, global_step = 160, loss = 4.81324
INFO:tensorflow:Create CheckpointSaverHook.
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-160
INFO:tensorflow:Saving checkpoints for 161 into cifar10_model\model.ckpt.
INFO:tensorflow:train_accuracy = 0.492188, cross_entropy = 1.34392, learning_rate = 0.1
INFO:tensorflow:step = 161, loss = 1.55667
INFO:tensorflow:Saving checkpoints for 200 into cifar10_model\model.ckpt.
INFO:tensorflow:Loss for final step: 1.5797.
INFO:tensorflow:Starting evaluation at 2017-12-12-01:29:05
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-200
INFO:tensorflow:Finished evaluation at 2017-12-12-01:29:14
INFO:tensorflow:Saving dict for global step 200: accuracy = 0.155446, global_step = 200, loss = 3.95206
WARNING:tensorflow:Input graph does not contain a QueueRunner. That means predict yields forever. This is probably a mistake.
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-200
2017-12-12 06:43:11.379269: I C:\tf_jenkins\home\workspace\rel-win\M\windows\PY\35\tensorflow\core\platform\cpu_feature_guard.cc:137] Your CPU supports instructions that this TensorFlow binary was not compiled to use: AVX AVX2


==> figures/results/CNNs/RESNET/Cifar10/OrigCode_(nonBuggy)/MR1-permutingRGB/Training/5Epochs/logs_MR1_GBR_5epochs <==
INFO:tensorflow:Using config: {'_num_worker_replicas': 1, '_tf_random_seed': 7, '_is_chief': True, '_task_type': 'worker', '_master': '', '_save_summary_steps': 100, '_service': None, '_num_ps_replicas': 0, '_keep_checkpoint_every_n_hours': 10000, '_log_step_count_steps': 100, '_model_dir': 'cifar10_model', '_cluster_spec': <tensorflow.python.training.server_lib.ClusterSpec object at 0x0000020ABE45FAC8>, '_save_checkpoints_steps': None, '_save_checkpoints_secs': 1000000000.0, '_session_config': None, '_task_id': 0, '_keep_checkpoint_max': 5}
WARNING:tensorflow:From codeWithMRs/MR1-changeRGB/cifar10_main_VERML_basedOn_nas_fix4_deterministic_gbr.py:87: FixedLengthRecordDataset.__init__ (from tensorflow.contrib.data.python.ops.readers) is deprecated and will be removed in a future version.
Instructions for updating:
Use `tf.data.FixedLengthRecordDataset`.
WARNING:tensorflow:From codeWithMRs/MR1-changeRGB/cifar10_main_VERML_basedOn_nas_fix4_deterministic_gbr.py:166: calling Dataset.map (from tensorflow.contrib.data.python.ops.dataset_ops) with output_buffer_size is deprecated and will be removed in a future version.
Instructions for updating:
Replace `num_threads=T` with `num_parallel_calls=T`. Replace `output_buffer_size=N` with `ds.prefetch(N)` on the returned dataset.
WARNING:tensorflow:From codeWithMRs/MR1-changeRGB/cifar10_main_VERML_basedOn_nas_fix4_deterministic_gbr.py:166: calling Dataset.map (from tensorflow.contrib.data.python.ops.dataset_ops) with num_threads is deprecated and will be removed in a future version.
Instructions for updating:
Replace `num_threads=T` with `num_parallel_calls=T`. Replace `output_buffer_size=N` with `ds.prefetch(N)` on the returned dataset.
INFO:tensorflow:Create CheckpointSaverHook.
INFO:tensorflow:Saving checkpoints for 1 into cifar10_model\model.ckpt.
INFO:tensorflow:cross_entropy = 2.6737, learning_rate = 0.1, train_accuracy = 0.0703125
INFO:tensorflow:loss = 2.88577, step = 1
INFO:tensorflow:Saving checkpoints for 40 into cifar10_model\model.ckpt.
INFO:tensorflow:Loss for final step: 2.19825.
INFO:tensorflow:Starting evaluation at 2017-12-11-13:33:39
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-40
INFO:tensorflow:Finished evaluation at 2017-12-11-13:33:48
INFO:tensorflow:Saving dict for global step 40: accuracy = 0.125743, global_step = 40, loss = 92.8017
INFO:tensorflow:Create CheckpointSaverHook.
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-40
INFO:tensorflow:Saving checkpoints for 41 into cifar10_model\model.ckpt.
INFO:tensorflow:cross_entropy = 1.77578, learning_rate = 0.1, train_accuracy = 0.289063
INFO:tensorflow:loss = 1.98933, step = 41
INFO:tensorflow:Saving checkpoints for 80 into cifar10_model\model.ckpt.
INFO:tensorflow:Loss for final step: 2.06074.
INFO:tensorflow:Starting evaluation at 2017-12-11-13:36:57
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-80
INFO:tensorflow:Finished evaluation at 2017-12-11-13:37:06
INFO:tensorflow:Saving dict for global step 80: accuracy = 0.107921, global_step = 80, loss = 47.5707
INFO:tensorflow:Create CheckpointSaverHook.
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-80
INFO:tensorflow:Saving checkpoints for 81 into cifar10_model\model.ckpt.
INFO:tensorflow:cross_entropy = 1.63527, learning_rate = 0.1, train_accuracy = 0.359375
INFO:tensorflow:loss = 1.84856, step = 81
INFO:tensorflow:Saving checkpoints for 120 into cifar10_model\model.ckpt.
INFO:tensorflow:Loss for final step: 1.86958.
INFO:tensorflow:Starting evaluation at 2017-12-11-13:40:11
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-120
INFO:tensorflow:Finished evaluation at 2017-12-11-13:40:20
INFO:tensorflow:Saving dict for global step 120: accuracy = 0.110891, global_step = 120, loss = 9.45242
INFO:tensorflow:Create CheckpointSaverHook.
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-120
INFO:tensorflow:Saving checkpoints for 121 into cifar10_model\model.ckpt.
INFO:tensorflow:cross_entropy = 1.51953, learning_rate = 0.1, train_accuracy = 0.398438
INFO:tensorflow:loss = 1.73213, step = 121
INFO:tensorflow:Saving checkpoints for 160 into cifar10_model\model.ckpt.
INFO:tensorflow:Loss for final step: 1.75286.
INFO:tensorflow:Starting evaluation at 2017-12-11-13:43:26
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-160
INFO:tensorflow:Finished evaluation at 2017-12-11-13:43:35
INFO:tensorflow:Saving dict for global step 160: accuracy = 0.121782, global_step = 160, loss = 5.88101
INFO:tensorflow:Create CheckpointSaverHook.
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-160
INFO:tensorflow:Saving checkpoints for 161 into cifar10_model\model.ckpt.
INFO:tensorflow:cross_entropy = 1.40018, learning_rate = 0.1, train_accuracy = 0.453125
INFO:tensorflow:loss = 1.61269, step = 161
INFO:tensorflow:Saving checkpoints for 200 into cifar10_model\model.ckpt.
INFO:tensorflow:Loss for final step: 1.73473.
INFO:tensorflow:Starting evaluation at 2017-12-11-13:46:39
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-200
INFO:tensorflow:Finished evaluation at 2017-12-11-13:46:48
INFO:tensorflow:Saving dict for global step 200: accuracy = 0.194059, global_step = 200, loss = 2.97268
WARNING:tensorflow:Input graph does not contain a QueueRunner. That means predict yields forever. This is probably a mistake.
INFO:tensorflow:Restoring parameters from cifar10_model\model.ckpt-200
2017-12-11 19:00:43.861336: I C:\tf_jenkins\home\workspace\rel-win\M\windows\PY\35\tensorflow\core\platform\cpu_feature_guard.cc:137] Your CPU supports instructions that this TensorFlow binary was not compiled to use: AVX AVX2


==> figures/results/CNNs/RESNET/Cifar10/OrigCode_(nonBuggy)/MR1-permutingRGB/stddevDevTesting <==
Testing\150Epochs\combinedData.csv,1.22708,0.0253447


==> figures/results/CNNs/RESNET/Cifar10/OrigCode_(nonBuggy)/MR1-permutingRGB/stddevDevTraining <==
Training\150Epochs\combinedData.csv,0.0243882,0.00946705


==> figures/results/CNNs/RESNET/Cifar10/OrigCode_(nonBuggy)/MR2-permutingConvOrder/stddevDevTesting <==
Testing\150Epochs\combinedData.csv,0.962114,0.01855


==> figures/results/CNNs/RESNET/Cifar10/OrigCode_(nonBuggy)/MR2-permutingConvOrder/stddevDevTraining <==
Training\150Epochs\combinedData.csv,0.0483508,0.0226901

